When Sensitivity Bias Varies Across Subgroups: The Impact of Non-uniform Polarity in List Experiments

Survey researchers face the problem of sensitivity bias: since people are reluctant to reveal socially undesirable or otherwise risky traits, aggregate estimates of these traits will be biased. List experiments offer a solution by conferring respondents greater privacy. However, little is know about how list experiments fare when sensitivity bias varies across respondent subgroups. For example, a trait that is socially undesirable to one group may socially desirable in a second group, leading sensitivity bias to be negative in the first group, while it is positive in the second. Or a trait may be not sensitive in one group, leading sensitivity bias to be zero in one group and non-zero in another. We use Monte Carlo simulations to explore what happens when the polarity (sign) of sensitivity bias is non-uniform. We find that a general diagnostic test yields false positives and that commonly used estimators return biased estimates of the prevalence of the sensitive trait, coefficients of covariates, and sensitivity bias itself. The bias is worse when polarity runs in opposite directions across subgroups, and as the difference in subgroup sizes increases. Significantly, non-uniform polarity could explain why some list experiments appear to 'fail'. By defining and systematically investigating the problem of non-uniform polarity, we hope to save some studies from the file-drawer and provide some guidance for future research.

==> _extensions/mikemahoney218/arxiv/partials/_authors.tex <==
$-- You can use as many custom partials as you need. Convention is to prefix name with '_'
$-- It can be useful to use such template to split some template parts in smaller pieces, which is easier to reuse.
$-- This '_custom.tex' is used on 'title.tex' as example.
$-- See other existing format in quarto-journals/ organisation.
$-- %%%% TODO %%%%%
$-- Use it if you need to insert content at this specific place of the main Pandoc's template. Otherwise, remove it.
$-- Here we are using it to format the authors part of the template.
$-- %%%%%%%%%%%%%%%
\textbf{$it.name.literal$}$if(it.orcid)$~\orcidlink{$it.orcid$}$endif$$for(it.affiliations/first)$\\$it.department$\\$it.name$\\$if(it.city)$$it.city$$if(it.postal-code)$,\ $it.postal-code$$endif$$endif$$endfor$\\$if(it.email)$\href{mailto:$it.email$}{$it.email$}$endif$


==> _extensions/mikemahoney218/arxiv/partials/before-body.tex <==
$-- Implements the frontmatter, title page, and abstract.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, otherwise remove this partials to use Quarto default one
$-- %%%%%%%%%%%%%%%%
$if(has-frontmatter)$
\frontmatter
$endif$
$if(title)$
$if(beamer)$
\frame{\titlepage}
$else$
\maketitle
$endif$
$if(abstract)$
\begin{abstract}
$abstract$
\end{abstract}
$endif$
$endif$
$if(keywords)$
{\bfseries \emph Keywords}
\def\sep{\textbullet\ }
$for(keywords/allbutlast)$$keywords$ \sep $endfor$
$for(keywords/last)$$keywords$$endfor$

$endif$


==> _extensions/mikemahoney218/arxiv/partials/title.tex <==
$-- Provides configuration of document metadata for writing the title block.
$-- Note that in addition to these templates and partials, Quarto will also make normalized authors and affiliations data available to the template,
$-- making is easy to write custom title blocks against a standard schema.
$--
$-- %%%% TODO %%%%%
$-- Customize is needed, like below for printing the authors. Otherwise remove this partials to use Quarto default one.
$-- %%%%%%%%%%%%%%%%
$if(linenumbers)$
\usepackage{lineno}
\linenumbers
$endif$
$if(doublespacing)$
\usepackage{setspace}
\doublespacing
$endif$
$if(date)$
\renewcommand{\today}{$date$}
$endif$
\newcommand{\runninghead}{A Preprint }
$if(runninghead)$
\renewcommand{\runninghead}{$runninghead$ }
$endif$
$if(title)$
\title{$title$$if(thanks)$\thanks{$thanks$}$endif$}
$endif$
$if(subtitle)$
\usepackage{etoolbox}
\makeatletter
\providecommand{\subtitle}[1]{% add subtitle to \maketitle
  \apptocmd{\@title}{\par {\large #1 \par}}{}{}
}
\makeatother
\subtitle{$subtitle$}
$endif$
\def\asep{\\\\\\ } % default: all authors on same column
$if(authorcols)$
\def\asep{\And }
$endif$
\author{${ by-author:_authors.tex()[\asep] }}
\date{$date$}

